Fast American Option Pricing using Nonlinear Stencils

We study the binomial, trinomial, and Black-Scholes-Merton models of option pricing. We present fast parallel discrete-time finite-difference algorithms for American call option pricing under the binomial and trinomial models and American put option pricing under the Black-Scholes-Merton model. For $T$-step finite differences, each algorithm runs in $O(\left(T\log^2{T}\right)/p + T)$ time under a greedy scheduler on $p$ processing cores, which is a significant improvement over the $\Theta({T^2}/{p}) + \Omega(T\log{T})$ time taken by the corresponding state-of-the-art parallel algorithm. Even when run on a single core, the $O(T\log^2{T})$ time taken by our algorithms is asymptotically much smaller than the $\Theta(T^2)$ running time of the fastest known serial algorithms. Implementations of our algorithms significantly outperform the fastest implementations of existing algorithms in practice, e.g., when run for $T \approx 1000$ steps on a 48-core machine, our algorithm for the binomial model runs at least $15\times$ faster than the fastest existing parallel program for the same model with the speed-up factor gradually reaching beyond $500\times$ for $T \approx 0.5 \times 10^6$. It saves more than 80\% energy when $T \approx 4000$, and more than 99\% energy for $T > 60,000$. Our option pricing algorithms can be viewed as solving a class of nonlinear 1D stencil (i.e., finite-difference) computation problems efficiently using the Fast Fourier Transform (FFT). To our knowledge, ours are the first algorithms to handle such stencils in $o(T^2)$ time. These contributions are of independent interest as stencil computations have a wide range of applications beyond quantitative finance.

==> 2-background.tex <==
\section{Background and Related Work}

%In the option pricing theory, options are contracts that give the right to buy or sell a security at a strike price on or before an expiration day. depending on the right of options, there are two types of options: call and put. A call option gives the right to buy and a put option gives the right to sell. Depending on the expiration date and rule for settlement, there are two styles of options: European and American. A European option can only be exercised at the expiration date and an American option can be exercised at any time before the expiration date. 
% Option contracts traded on futures exchanges are mainly American-style, whereas those traded over the counter are mainly European.
%The theoretical value of an option is determined by stock price, exercise price, volatility, interest rate, and time to expiration.

% European option pricing in O(1) time.

% \subsection{Option pricing models}

%The earliest option pricing model \cite{bachelier1900theorie,samuelson2011louis} and its extensions \cite{black1973pricing, merton1973theory} are based on the assumption of the geometric Brownian motion for asset pricing and the no-arbitrage idea.
\hide{
\textbf{Option Pricing Model}: The earliest option pricing model \cite{bachelier1900theorie,samuelson2011louis} and its extensions \cite{black1973pricing, merton1973theory} are based on the assumption of the geometric Brownian motion for asset pricing and the no-arbitrage idea. This strategy uses lognormal distribution and is inconsistent with real-world skewed distribution. Subsequent research resolved the inconsistency using state and time-dependent \cite{derman1998stochastic, dupire1994pricing} and stochastic \cite{stein1991stock, heston1993closed, ball1994stochastic,bergomi2015stochastic} volatility models, jump diffusions models \cite{merton1976option, kou2002jump, bakshi2000spanning, duffie2000transform, dempster2002spread,matsuda2004introduction,runggaldier2003jump}, pure jump model (variance-gamma process) \cite{madan1998variance}, Lévy processes based models \cite{geman2001time, jackson2008fourier}, and binomial model \cite{derman1994riding, dupire1994pricing}. 
}
% hide ends

\noindent\textbf{FFT methods in Finance}: The Fourier Transform method is widely used in solving differential equations \cite{kerr1988namias,le1972use,evans2010partial}, probability and statistics \cite{pinelis2015characteristic,schatte1988strong} (in probability theory, the characteristic function \cite{polya1949remarks} is the Fourier transform of the probability density function), and signal processing \cite{brandwood2012fourier,orfanidis1995introduction}. More specifically, Fourier transforms can be used to find the integral form solutions of parabolic Partial Differential Equations (PDEs) under infinite domain constraint \cite{ockendon2003applied,evans2010partial}. Black, Scholes, and Merton \cite{black1973pricing,merton1973theory} showed that the European option can be calculated by the Black-Scholes-Merton formula, %which is 
a parabolic PDE with infinite domain constraint. Hence, the Fourier Transform yields an integral form for the European option.
%by using the Fourier Transform, one gets an integral form for the European option. 
However, to get the numerical value from the integral form one uses numerical integration \cite{hildebrand1987introduction,burden2015numerical} which can be sped up by FFT algorithm. FFT-based approaches for numerical integration have been used in other models as well, such as applying the jump-diffusion-based Black-Scholes model \cite{zhang2012fast} to Black-Scholes Model for American options \cite{chang2007richardson,oliveira2014convolution,zhylyevskyy2010fast,lord2008fast}. However, those methods rely heavily on mathematical theory, do not apply to the binomial model, need to know the analytical form of the characteristic function, and are restricted to the infinite domain problem \cite{cont2005finite}. 
    %For example, the repeated Richardson extrapolation method \cite{chang2007richardson,oliveira2014convolution,zhylyevskyy2010fast}, when repeated $k$ times, takes $\Om{ k^2 T^2 \log T }$ time with arithmetically decreasing step sizes and $\Om{ 2^k T^2 \log T }$ time with geometrically decreasing step sizes. See the appendix for details.

\hide{
\noindent\textbf{Monte Carlo methods}: For a model incapable of computing the option price in closed form, an alternative way is to use Monte Carlo methods \cite{duan1998empirical}, which rely on the probabilistic characterization of the model. The Monte Carlo methods are hard to develop for some options, such as Black-Scholes Model for the American put option, which will need to determine the Early Exercise Boundary simultaneously, but there are still many results on Monte Carlo Methods \cite{ibanez2004monte,longstaff2001valuing,tsitsiklis2001regression,boyle1977options}.
}
% hide ends

\hide{
\noindent\textbf{Finite Difference method}: For a model that can be formulated as PDEs, one can use the finite difference method to discretize the PDEs and formulate it as a stencil computation problem. The finite difference method is easy to formulate and has guaranteed convergence results; However, the na\"ive way of performing the stencil computation requires $\Oh{T^2}$ time, where $T$ is the number of time steps. Inspired by the results in \cite{ahmad2021fast, ahmad2022fourst}, which show that $T$ time steps of a linear stencil computation on a one-dimensional input grid of length $\Th{T}$ take $\Oh{T \log^2 T}$ time, we show how a class of nonlinear stencil computations can be performed in $\Oh{T \log^2 T}$ time as well. More specifically, we design an FFT-based algorithm to solve the stencil computation problem obtained by discretizing the Black-Scholes PDE for the American put option, which requires $\Oh{ T \log^2 T }$ time and achieves $\Oh{\frac{1}{T}}$ global error \cite{thomas2013numerical}. In addition, since the binomial model already poses the American call option pricing problem as a stencil computation problem, we can solve the binomial-tree-based American call option in $\Oh{ T \log^2 T }$ time as well. 
}
% hide ends

\hide{
\noindent\textbf{Algorithms for stencil computations}: There are several algorithms to solve  stencil computation problems. The first category is standard algorithms that perform stencil computations by repeatedly applying the stencil operator iteratively on the evolving data. The class includes looping algorithms, tiled looping algorithms \cite{Bandishti2012, bondhugula2017,Wolfe1987,Wolf1991,Wolf1996,Wonnacott2002,bondhugula2016plutoplus,Andonov1997,Hogstedt1999, Zhang2015A3D, Malas2014TowardsEE,Malas2015}, and recursive divide-and-conquer algorithms \cite{frigo2005cache, FrigoSt2009, tang2011pochoir, Ekanathan2017, Katsuto2010, Sriram2007}. All these algorithms 
    work for both linear and nonlinear stencils in arbitrary dimensions under periodic and boundary conditions, but differ in the way to apply the stencil.
    They have the same computational complexity of $\Th{NT}$ where $N$ is the size of the grid. Recently, Ahmad et al. \cite{ahmad2021fast} presented an FFT-based algorithm that is the first algorithm to perform linear stencil computations in $\oh{NT}$ computational complexity.
}
% hide ends
    
